Zero-th Order Algorithm for Softmax Attention Optimization

Large language models (LLMs) have brought about significant transformations in human society. Among the crucial computations in LLMs, the softmax unit holds great importance. Its helps the model generating a probability distribution on potential subsequent words or phrases, considering a series of input words. By utilizing this distribution, the model selects the most probable next word or phrase, based on the assigned probabilities. The softmax unit assumes a vital function in LLM training as it facilitates learning from data through the adjustment of neural network weights and biases. With the development of the size of LLMs, computing the gradient becomes expensive. However, Zero-th Order method can approximately compute the gradient with only forward passes. In this paper, we present a Zero-th Order algorithm specifically tailored for Softmax optimization. We demonstrate the convergence of our algorithm, highlighting its effectiveness in efficiently computing gradients for large-scale LLMs. By leveraging the Zeroth-Order method, our work contributes to the advancement of optimization techniques in the context of complex language models.

==> previous.tex <==
\section{Previous Results from \texorpdfstring{\cite{mgn+23}}{}}

\Yichuan{Most things in this section will be finally removed}

\subsection{Descent Lemma}

% \Zhao{You need to show softmax loss is $\ell$-smooth, then you can apply}\Yichuan{done in Section~\ref{sec:softmax_smooth}}
\begin{lemma}[Lemma~1 in \cite{mgn+23}, \Yichuan{Can be used for Softmax directly}]
    Let $L(x)$ be an $\ell$-smooth function, then for any unbiased gradient estimate $\wh{g}$, it holds that
    \begin{align*}
        \E[L(x_{t+1}) ~|~ x_t] - L(x_t) \le - \eta \cdot \|\nabla L(x_t)\|^2 + \frac{1}{2} \eta^2 \ell \cdot \E[\|\wh{g}(x, \mathcal{B})\|^2]
    \end{align*}
\end{lemma}

\subsection{Gradient Bound}


\subsection{Convergence Rate (Dimension-Free)}

\begin{assumption}[Local $r$-effective Rank]
\label{ass:effect_rank}
    Let $G(x_t) = \max_{(a, b) \in \mathcal{D}}\|\nabla L(x_t; \{(a, b)\})\|$. There exists a matrix $H(x_t)$ such that,
    \begin{enumerate}
        \item For any $x$ such that $\|x - x_t\| \le \eta d G(x_t)$, it holds that $\nabla^2 L(x) \preceq H(x_t)$, where $\nabla^2 L(x)$ denotes the Hessian on all data points; 
        \item The effective rank of $H(x_t)$ is bounded by $r$, i.e.,
        \begin{align*}
            \tr[H(x_t)]/\|H(x_t)\|_{\mathrm{op}} \le r. 
        \end{align*}
    \end{enumerate}
\end{assumption}

\begin{lemma}[Convergence Rate, Theorem~1 in \cite{mgn+23}]
\label{lem:converge_rate}
    Let $x_{t+1} \gets x_t - \eta \wh{g}(x_t)$, where $\wh{g}(x_t)$ is computed with respect to the batch $\mathcal{B}$. Consider $L(x)$ has the property of $r$-effective rank (Assumption~\ref{ass:effect_rank}), then there exists a parameter $\gamma = \Theta(r/n)$ such that the expected loss decrease can be bounded as \Yichuan{I think we can directly compute the effective rank of softmax function, so that we can replace the $\gamma$ here}
    \begin{align*}
        \E[L(x_{t+1} ) |x_t] - L(x_t) \le -\eta \|\nabla L(x_t)\|^2 \frac{1}{2} \eta^2 \ell \cdot \gamma \cdot \E[\|\nabla L(x; \mathcal{B})\|^2]
    \end{align*}
\end{lemma}

\begin{remark}
    The choice of $\gamma$ is 
    \begin{align*}
        \gamma = \frac{dr + d - 2}{n(d + 2)} + 1
    \end{align*}
\end{remark}

\subsection{Properties of Gaussian Purterbations}




\begin{lemma}[Lemma~5 in \cite{mgn+23}]
\label{lem:prop_gauss}
    Let $z \in \R^n$ with $z_i \sim \N(0, 1)$ i.i.d. Then it holds that
    \begin{align*}
       &~ \E[\wh{g}(x, \mathcal{B})\wh{g}(x, \mathcal{B})^\top] \\
    =  &~ (1+\frac{1}{n})\cdot (\nabla L(x)L(x)^\top +\frac{1}{B}\Sigma _{MB}(x)) + \frac{1}{n}I\cdot (\|\nabla L(x)\|^2 + \frac{1}{B}\tr(\Sigma _{MB}(x))). 
    \end{align*}
\end{lemma}


\begin{proof}[Proof for Lemma~\ref{lem:converge_rate}]
    By Taylor’s theorem with remainder, we have that
    \begin{align*}
        L(x_{t+1})
    = &~L(x_{t}) +\nabla L(x_t)^\top (x_{t+1} - x_t)\\
      &~ + \int_{0}^1 \lambda(x_{t+1} - x_t)^\top \nabla^2L(\lambda x_{t+1} + (1 - \lambda)x_t)(x_{t+1} - x)^\top d\lambda.
    \end{align*}
    Then by 
    \begin{align*}
        \|x_{t+1} - x_t\| 
    = &~\eta \cdot \|\wh{g}(x; \mathcal{B})\| \\
    \le&~\eta \sqrt{d} \cdot \frac{1}{nB}\sum |z_i^\top \nabla L(x;\{(x, y)\})| \\
    \le&~\eta d G(x_t).
    \end{align*}
    Thus we have
    \begin{align*}
        \|\lambda x_{t+1} +(1 - \lambda)x_t - x_t\| \le \eta d G(x_t).
    \end{align*}
    By the assumption we have the upper bound
    \begin{align*}
        \nabla^2 L(\lambda x_{t+1} +(1 - \lambda)x_t) \preceq H(x_t),
    \end{align*}
    we have
    \begin{align*}
        L(x_{t+1}) 
    \le &~ L(x_t) +\nabla L(x_t)^\top (x_{t+1} - x_t) + (x_{t+1} - x_t)^\top H(x_t)(x_{t+1} - x_t) \\
    = &~ L(x_t) - \eta \nabla L(x_t)^\top \wh{g}(x_t;\mathcal{B}) + \frac{1}{2}\eta^2 \wh{g}(x_t;\mathcal{B})^\top H(x_t)\wh{g}(x_t; \mathcal{B}).
    \end{align*}
    Taking conditional expectation with respect to $x_t$ and plugging Lemma~\ref{lem:prop_gauss}, we have
    \begin{align*}
        \E[L(x_{t+1})|x_t]
    \le &~ L(x_t) - \eta \|\nabla L(x_t)\|^2 +\frac{\eta^2}{2} \langle H(x_t), \E[\wh{g}(x;\mathcal{B})\wh{g}(x;\mathcal{B})^\top] \rangle \\
    = &~ L(x_t) - \eta \|\nabla L(x_t)\|^2 + \frac{\eta^2}{2} \cdot \frac{d}{n(n(d+2))} \cdot (\|\nabla L(x_t)\|^2 + \frac{1}{B} \tr(\Sigma(x_t)))\tr(H(x_t)) \\
    &~+ \frac{\eta^2}{2}(1 + \frac{d-2}{n(d+2)})(\nabla L(x_t)^\top H(x_t)\nabla L(x_t) + \frac{1}{B}\langle \Sigma(x_t), H(x_t)\rangle).
    \end{align*}
    By assumption, the Hessian upper bound $H(x_t)$ satisfies $\|H(x_t)\|_{\mathrm{op}} \le \ell$ and $\tr(H(x_t)) \le \ell r$. \Yichuan{This is where they use the effective rank.}Then we have
    \begin{align*}
        \E[L(x_{t+1})|x_t]
    \le &~ L(x_t) - \eta \|\nabla L(x_t)\|^2 + \frac{\eta^2 \ell}{2} \cdot (\frac{dr+d-2}{n(d+2)} + 1)\cdot (\|\nabla L(x_t)\|^2 + \frac{1}{B} \tr(\Sigma(x_t)) \\
    = &~ L(x_t) - \eta \|\nabla L(x_t)\|^2 + \frac{\eta^2 \ell}{2} \cdot \E[\|\nabla L(x_t;\mathcal{B})\|^2].
    \end{align*}

    Thus we complete the proof
\end{proof}
